Low-Rank Nonlinear Decoding of $\mu$-ECoG from the Primary Auditory Cortex

This paper considers the problem of neural decoding from parallel neural measurements systems such as micro-electrocorticography ($\mu$-ECoG). In systems with large numbers of array elements at very high sampling rates, the dimension of the raw measurement data may be large. Learning neural decoders for this high-dimensional data can be challenging, particularly when the number of training samples is limited. To address this challenge, this work presents a novel neural network decoder with a low-rank structure in the first hidden layer. The low-rank constraints dramatically reduce the number of parameters in the decoder while still enabling a rich class of nonlinear decoder maps. The low-rank decoder is illustrated on $\mu$-ECoG data from the primary auditory cortex (A1) of awake rats. This decoding problem is particularly challenging due to the complexity of neural responses in the auditory cortex and the presence of confounding signals in awake animals. It is shown that the proposed low-rank decoder significantly outperforms models using standard dimensionality reduction techniques such as principal component analysis (PCA).

==> low_rank_model.tex <==
\begin{figure}[t]\centering
\scalebox{0.25}{
\begin{tikzpicture}[thick,->,draw=black!80, node distance=2.5cm, scale=1, every node/.style={scale=1.5, font=\large}]
\tikzstyle{every pin edge}=[<-,line width=3pt]
\tikzstyle{neuron}=[circle,fill=black!25,minimum size=30pt,inner sep=0pt]

\tikzstyle{lowrank neuron}=[circle,fill=black!25,minimum size=55pt,inner sep=0pt, fill=yellow!20];

\tikzstyle{hidden neuron}=[neuron, fill=red!30];

\tikzstyle{annot} = [text width=1em, text centered]
\tikzstyle{null} = [draw = none , fill= none]
\tikzstyle{line} = [draw, black, -latex']
\tikzstyle{X block}=[rectangle,draw=blue!65,fill=blue!25,minimum size=40pt, minimum height=3cm,minimum width=4cm]

\tikzstyle{Z block}=[rectangle,draw=green!65, fill=green!35,minimum size=40pt, minimum height=3cm,minimum width=1.5cm]

\tikzstyle{V}=[rectangle,fill=cyan!25,minimum size=4pt, minimum height=1cm,minimum width=2mm]

\tikzstyle{U}=[rectangle,fill=black!25,minimum size=4pt, minimum height=2mm,minimum width=1cm]

\node[rectangle, fill = black!5, draw=black!20, minimum width = 13.5cm , minimum height= 9cm, rounded corners=5mm, xshift = 9.5cm, yshift = 0.25cm](model){};

\node[annot, above of = model, yshift = 2.5cm, text width = 10cm, font=\LARGE]{Low-Rank Decoder};

\node[X block, font=\LARGE](X){$\mathbf{X}$};
\node[annot, above of = X, yshift = -0.7cm, xshift = -0.3cm, font=\LARGE](input){input};
\node[annot, below of = X, yshift = 0.7cm, xshift = -0.3cm, font=\LARGE]{time};
\node[annot, left of = X, xshift = 0.2cm,yshift = 0cm, font=\LARGE]{d};

%\node[xshift = -3.5cm, yshift=-.3cm,left of = X] (rat) 
%    {\includegraphics[scale = 0.2]{rat_array-1.png}};


\node[Z block, right of= X, xshift = 3cm, font=\LARGE](Z){$\mathbf{Z}_0$};
\node[annot, below of = Z, yshift = 0.7cm, font=\LARGE]{freq};
\node[annot, left of = Z, yshift = 0cm, xshift = 1.5cm, font=\LARGE](d){d};


\path (X) edge [above, line width=0.8mm, draw=black!50] node[text width = 4em, xshift = 0.5cm, font=\LARGE]{DCT}(d);

\node [lowrank neuron, right of = Z, yshift = 2.9cm, xshift = 1cm, font=\LARGE] (l1){$\quad \mathbf{v}_1 \mathbf{u}_1\tran$};
\node[V, right of=Z, xshift = 0.5cm, yshift = 3cm, font=\LARGE](v1){};
\node[U, right of=Z, xshift = 1.2cm, yshift = 3.4cm, font=\LARGE](u1){};

\node [lowrank neuron, below of = l1, yshift = 0.3cm, font=\LARGE] (l2) {$\quad \mathbf{v}_2 \mathbf{u}_2\tran$};
\node[V, right of=Z, xshift = 0.5cm, yshift = 0.8cm, font=\LARGE](v2){};
\node[U, right of=Z, xshift = 1.2cm, yshift = 1.2cm, font=\LARGE](u2){};

\node[annot, below of = l2, yshift = 0.7cm ]{$\vdots$};

\node [lowrank neuron, below of = l2, yshift = -1cm, font=\LARGE] (l3) {$\quad \mathbf{v}_3 \mathbf{u}_3\tran$};
\node[V, right of=Z, xshift = 0.5cm, yshift = -2.7cm, font=\LARGE](v3){};
\node[U, right of=Z, xshift = 1.2cm, yshift = -2.3cm, font=\LARGE](u3){};



\path (Z) edge [above, line width=0.6mm, draw=black!50] (l1);
\path (Z) edge [above, line width=0.6mm, draw=black!50] (l2);
\path (Z) edge [above, line width=0.6mm, draw=black!50] (l3);

\node [hidden neuron, right of = l1, xshift = 1cm, yshift = -.5cm, font=\LARGE] (h1) {$\sigma$};
\node [hidden neuron, below of = h1, yshift = 0.9cm, font=\LARGE] (h2) {$\sigma$};
\node[annot, below of = h2, yshift = 0.9cm ](dots){$\vdots$};
\node [hidden neuron, below of = dots, yshift = 1cm, font=\LARGE] (h3) {$\sigma$};

\foreach \j in {1,2,3}
    \foreach \i in {1,2,3}
        \path (l\i) edge (h\j);

\node [hidden neuron, right of = h2, yshift = -1cm, xshift = 0cm, font=\LARGE] (out) {$\sigma$};

\foreach \i in {1,2,3}
        \path (h\i) edge (out);
\node [null, right of=out, font=\LARGE](y){};
\path (out) edge [right, line width=0.8mm, draw=black!50] node[text width = 4em, xshift=1.5cm, font=\LARGE]{$\mathbf{y}$}(y);

\node[annot, above of = y, yshift = -1.5cm, xshift = 0.3cm, font=\LARGE]{output};
\node[annot, right of=l1, yshift = 0.7cm, xshift = -0.5cm, font=\LARGE]{$\mathbf{W}_2$};
\node[annot, right of=h1, yshift = -0.8cm, xshift = -0.7cm, font=\LARGE]{$\mathbf{w}_3$};
\end{tikzpicture}
}
\caption{Schematic of the model used for decoding of a multidimensional neural process.\label{fig:LowR}} 
\end{figure}







